Learning a self-supervised tone mapping operator via feature contrast masking loss

High Dynamic Range (HDR) content is becoming ubiquitous due to the rapid development of capture technologies. Nevertheless, the dynamic range of common display devices is still limited, therefore tone mapping (TM) remains a key challenge for image visualization. Recent work has demonstrated that neural networks can achieve remarkable performance in this task when compared to traditional methods, however, the quality of the results of these learning-based methods is limited by the training data. Most existing works use as training set a curated selection of best-performing results from existing traditional tone mapping operators (often guided by a quality metric), therefore, the quality of newly generated results is fundamentally limited by the performance of such operators. This quality might be even further limited by the pool of HDR content that is used for training. In this work we propose a learning-based self-supervised tone mapping operator that is trained at test time specifically for each HDR image and does not need any data labeling. The key novelty of our approach is a carefully designed loss function built upon fundamental knowledge on contrast perception that allows for directly comparing the content in the HDR and tone mapped images. We achieve this goal by reformulating classic VGG feature maps into feature contrast maps that normalize local feature differences by their average magnitude in a local neighborhood, allowing our loss to account for contrast masking effects. We perform extensive ablation studies and exploration of parameters and demonstrate that our solution outperforms existing approaches with a single set of fixed parameters, as confirmed by both objective and subjective metrics.

==> EG22_body.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title{Self-supervised Tone Mapping Network with Feature Contrast Masking Loss}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[D. Fellner \& S. Behnke]
{\parbox{\textwidth}{\centering D.\,W. Fellner\thanks{Chairman Eurographics Publications Board}$^{1,2}$\orcid{0000-0001-7756-0901}
        and S. Behnke$^{2}$\orcid{0000-0001-5923-423X} 
%        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$TU Darmstadt \& Fraunhofer IGD, Germany\\
         $^2$Graz University of Technology, Institute of Computer Graphics and Knowledge Visualization, Austria
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

% uncomment for using teaser
% \teaser{
%  \includegraphics[width=\linewidth]{eg_new}
%  \centering
%   \caption{New EG Logo}
% \label{fig:teaser}
%}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract} 
%The Tone Mapping algorithm can compress the dynamic range of high dynamic images (HDR) to accurately display them on the standard monitor. In particular, with the rapid growth of deep learning, an increasing number of learning-based operators are being proposed. Though they may produce more pleasing results, there is still some deficiency. Mostly the learning-based algorithms treat the tone mapping as image translation task, they generate HDR-LDR training pairs and apply fully-supervision to optimise a network. In fact, there is no perfectly reasonable tone mapping label, so this training mode is unsuitable for tone mapping. Furthermore, their networks are too complicated. This paper proposes a self-supervision with visual masking loss tone mapping network, which doesn't need the label and use the HDR image itself as guidance. Our network has only eight convolution layers. First, the HDR image will be exposure-sampled into three different exposed-LDR images, which will be the network inputs. Then, we design an adaptive $\mu$ law to the HDR images for global contrast compression. For the optimization, we adjust VGG with applying visual masking on feature maps as the loss function to have a better local contrast control. We achieve better results both on objective and subjective evaluation on the test set.

The Tone Mapping algorithm can compress the dynamic range of high dynamic images (HDR) to accurately display them on the standard monitor. In particular, with the rapid growth of deep learning, an increasing number of learning-based operators are being proposed. However, most of the learning-based algorithms treat tone mapping as the image restoration task, they generate HDR-LDR training pairs manually or guided by metrics, and optimize the complicated network through a supervised approach. On the one hand, there are no perfectly reasonable tone mapping operators, so the label will restrict the results. On the other hand, tone mapping is an information-reducing task, a simple network will suffice. In this paper, we train a small self-supervision tone mapping network at test time, which only uses the HDR image itself as the label. Our network only has eight convolution layers. In particular, we analyze tone mapping from three aspects, the structural similarity with the HDR image, the contrast, and brightness. Based on this, first, the HDR image will be exposure-sampled into three different exposed LDR images as the inputs to keep all the information while compressing the dynamic range. And an adaptive $\mu$ law will be applied to the HDR images for better brightness and global contrast compression. Most importantly, we put forward a novel feature contrast masking loss based on perceptual loss, which is proved by experiments to have a good effect on local contrast control.  Our methods outperform other SOTA tone mapping operators, both of subjective and objective evaluation.

%The Tone Mapping algorithm can compress the dynamic range of high dynamic images (HDR) to accurately display them on the standard monitor. In particular, with the rapid growth of deep learning, an increasing number of learning-based operators are being proposed. However, most of the learning-based algorithms treat tone mapping as the image restoration task, they generate HDR-LDR training pairs manually or guided by metrics, and optimize the complicated network through a supervised approach. On the one hand, there are no perfectly reasonable tone mapping operators, so the label will restrict the results. On the other hand, tone mapping is an information-reducing task, a simple network will suffice. In this paper, we train a small self-supervision tone mapping network at test time, which only uses the HDR image itself as the label. Our network only has eight convolution layers. In particular, we analyze tone mapping from three aspects, the structural similarity with the HDR image, the contrast, and brightness. Based on this, first, the HDR image will be exposure-sampled into three different exposed LDR images as the inputs to keep all the information while compressing the dynamic range. And an adaptive $\mu$ law will be applied to the HDR images for better brightness and global contrast compression. For better structural fidelity and local contrast control, we adopt perceptual loss by applying a designed visual masking model to the feature maps as the loss function. Our methods outperform other SOTA tone mapping operators, both of subjective and objective evaluation.
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012

%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>=
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Collision detection}
\ccsdesc[300]{Hardware~Sensors and actuators}
\ccsdesc[100]{Hardware~PCB design and layout}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------
\section{Introduction}
\label{intro}
High Dynamic Range (HDR) images can reproduce real-world appearance by directly encoding wide luminance and color gamut ranges.
With a fast pace of developments in camera technology HDR image and video capturing becomes feasible even for ordinary users. 
Regrettably, limited dynamic range of existing displays precludes immediate use of HDR content, and the-so-called tone mapping is required to adapt such content to display capabilities.
While a variety of different application-dependent goals of tone mapping might be considered \cite{mantiuk2015ency},
typically preserving as much as possible the original scene appearance or overall pleasant look are the key factors.

%Image dynamic range (DR) is the ratio between the largest and smallest pixel values within an image. High Dynamic Range images (HDRI) have much more larger DR while can provide more information compared with  Low Dynamic Range images  (LDRI). %HDRI is first utilized by Debevec \cite{debevec2008recovering} as a lighting tool to make CG objects illuminated in an actual context. With the fast-growing camera technology in recent years, capturing HDR images becomes easier. However, the current mainstream display is still a standard monitor, which is designed for LDRI and cannot support the HDR feature. The same issue also appears in printers. Consequently, compressing the HDRI to LDRI, which is so-called tone mapping, is still an active research area.
 

Tone mapping has been developed for decades \cite{reinhard2010high,banterle2017advanced} but the performance of even the most prominent techniques strongly depends on the HDR image content and specific parameter settings. 
A great variance in subjective evaluation of different techniques \cite{ledda2005evaluation,yoshida2005perceptual,vcadik2008evaluation} % cadik06image_attributes, cadik07evaluation,  
clearly indicates that both specific algorithms as well as default parameter settings, as often proposed by their respective authors, do not generalize across the scenes.
Manual selection of a suitable algorithm and experience in fine tuning of its parameters might be required for high quality results.
This hinders smooth adoption of HDR technology and is the key obstacle in developing machine learning solutions as we discuss next.

%Traditional algorithms can be mainly divided into two categories, global and local models. The global tone mapping methods \cite{larson1997visibility} \cite{drago2003adaptive} \cite{jack1993tone} will apply a curve to the whole HDRIs to compress the dynamic range. The local methods \cite{reinhard2002photographic} \cite{durand2002fast} \cite{liang2018hybrid} \cite{shibata2016gradient} \cite{li2018clustering} \cite{shan2009globally} will take into consideration the weights of neighboring pixels, some methods use filters to decompose the HDRI into a base layer and detail layer and mainly compress the base layer while keeping the detail layer unchanged, and some make use of sliding window to obtain the local feature. On the one hand, the conventional tone mapping model cannot work well for all scenarios, on the other hand, the parameter setting is not user-friendly for non-expert users.

Recently, an increasing number of learning-based tone mapping methods have been proposed that show huge potential in terms of generality and quality with respect to their traditional algorithm-based predecessors. However, there still are some shortcomings. First of all, most learning-based models regard tone mapping as an image restoration task and optimize the network in a fully supervised manner, which requires high quality paired HDR and tone mapped training data. Typically Tone Mapping Quality Index (TMQI) \cite{yeganeh2012objective} is used to select best performing labels, which might not fully agree with manual selection and reduces reliability of such labels. In addition, since such methods treat  tone mapping as image restoration task,  they usually involve large scale networks. However, tone mapping is an information reducing process, which is somehow easier than image restoration. 
Motivated by this observation, we are seeking here for an alternative solution that reduces the network size and optimizes information reduction for a given HDR image content.


As image contrast is arguably one of the key cues while seeing and interpreting images by the Human Visual System (HVS) \cite{palmer1999vision}, in our tone mapping solution we aim at reproducing perceived contrast in HDR scenes that also assures structural fidelity by reproducing visible image details.
To this end, we propose a simple image-specific, self-supervised tone mapping network that is trained at the test time and does not require any data labeling.
The only training data is an input HDR image, and  key novelty in our approach is the loss function that directly compares  the HDR and tone mapped images content.
As involved signals are of different dynamic ranges, a direct computation of the loss in the feature space, as e.g., in perceptual VGG loss \cite{simonyan2014very,johnson2016perceptual}, might lead to unpredictable results. 
To alleviate those problems we transform the HDR content to make it more VGG network friendly by normalizing pixel values and improving their histogram.
Most importantly, we formulate a local contrast measure in the feature space, which as any contrast measure involves the ratio operation and this way to a great extent abstracts from the dynamic range difference.
Motivated by contrast perception literature we consider feature contrast masking in the presence of similar features in the near spatial neighborhood.
Likewise, we introduce a compressive non-linearity as a function of feature contrast magnitude, so that for lower magnitudes any departs in feature contrast are stronger penalized in the loss.   
This allows us to better preserve image details, but also gives the network more freedom in changing absolute magnitude of strong feature contrast, in particular, when in the image spatial neighborhood similar features are present.
As confirmed by objective and subjective metrics, our loss formulation leads to a good visual match between tone mapped image and its HDR counterpart, and overall pleasant image appearance for a single set of loss parameters. 
We will make our code public once the paper is accepted.


%The essence of tone mapping is displaying HDRI in a standard monitor as close as possible to the real scene. We address this problem from three perspectives: structural fidelity, contrast, and brightness. Specifically, we train an image-specific self-supervised tone mapping network at test time. The network is consists of an encoder, fusion module, and decoder. At first, since the HDRI is stored in linearity format, which is not satisfied with Human Visual System (HVS) and the dynamic range is far surpassed the LDRI's, directly taking the HDRI as input is unreasonable. Therefore, we first do exposure sampling for the input HDR image, producing three different exposure LDR images, which can retain all the HDR information. Then, the high-dimensional features are fused by the fusion module. At last, the decoder will transform the fused features to the LDR image. For the same reason, directly using HDRI as the label to optimize is illogical, to this end, we design an adaptive $\mu$ law for the HDR image to compress the dynamic range, which can lead to non-linearity and is satisfied with Human Visual System (HVS). The adaptive $\mu$ law has a great effect on the brightness and global contrast of the tone mapping results. The paramount thing is that we present a novel feature contrast masking loss based on the perceptual loss \cite{simonyan2014very} \cite{johnson2016perceptual} to control the local contrast, which is inspired with the visual masking theory. To the best of our knowledge, this is the first time that regulate the contrast in feature space. Different from the common perceptual loss, the novel visual masking model will be applied to the feature maps first, and then calculate the loss. In addition, perceptual loss has a better effect than $L_{1}$ loss for the structural fidelity after experiments.
 
%As for the loss function, we select perceptual loss, and the experiments can prove that perceptual loss is better than $L_{1}$ loss for the structural fidelity. 
%Furthermore, inspired by the visual masking theory, we put forward a visual masking model to the feature maps of perceptual loss to have good control for the local contrast. This is to say, different from the common perceptual loss, the novel visual masking model will be applied to the feature maps first, and then calculate the loss. 

%In this paper, we propose a small image-specific self-supervision tone mapping network, which doesn't need extra-label training data. Through three well-designed modules, multiply exposure inputs,  adaptive $\mu$-law, and feature contrast masking loss, we can have a good reproduction for HDRI in terms of structural fidelity, contrast, and brightness in LDR displays and printers. We have tested our method with 180 images from three different datasets, and our method outperforms the SOTA methods both objective and subjective metrics. In addition, despite our method is learning-based, it still allows changing the image appearance by manipulating the feature contrast masking model in the loss function. Once the training process is completed, no more parameters need to be set. We will make our code public once the paper is accepted.
%Since our network is an end-to-end algorithm, it doesn't need parameters setting once trained, which is more user-friendly.
%Contributions:
%\begin{itemize}
%\item Propose a light-weight self-supervison tone mapping with multiple exposure inputs network, which take use HDR itself as ground truth and corresponding multiple exposure LDRs as input, which doesn't need label annotation.
%\item Design an adaptive $\mu$-law to control the global contrast and visual masking loss to the local contrast.
%\item Experiments prove the effectiveness of our method, achieve better results for both objective and subjective evaluation.
%\end{itemize}
%\begin{itemize}
%\item Propose a small image-specific self-supervision tone mapping network.
%\item Design multiply exposure inputs, an adaptive $\mu$-law, and visual masking perceptual loss to handle the structural fidelity, contrast, and brightness.
%\item Our method achieves the best results both of objective and subjective evaluation on a large-scale test set.
%\end{itemize}

%The paper is organized as follows. Section 2 introduces the related work. Section 3 describes our motivations and proposed method in detail. In section 4, subjective and objective experiment results are presented and analyzed. Section 5 demonstrates several explorations of our methods. Finally, the limitation is discussed in section 6 and the conclusion is in section 7.
%-------------------------------------------------------------------------
\section{Related Work}
In this section, we summarize background research on contrast perception modeling, and then we discuss tone mapping techniques with emphasis on those that explicitly process contrast as well as those more recent that are learning based.
\label{related work}


\subsection{Contrast Perception Modeling}
%Contrast is arguably one of the key cues while seeing, interpreting, and understanding images by the Human Visual System (HVS) \cite{palmer1999vision}.
%The most common contrast definitions are Michelson contrast, Weber fraction, or logarithmic contrast (refer to \cite{mantiuk2006perceptual} for conversions between those contrast measures), but in the nutschell the ratio of two signals is always involved.
Image contrast perception is characterized by a strong non-linearity that allows for more extensive absolute changes of higher supra-threshold contrast magnitude than their lower near-threshold counterparts before such manipulation becomes noticeable  \cite{kingdom1996contrast}. This effect is called self-contrast masking \cite{daly2000visual}.  

Another important effect in contrast perception is visual masking \cite{legge1980contrast,foley1994human,watson1997model}, where the thresholds for lower contrast detection or higher contrast change discrimination might be strongly elevated when in the close neighborhood contrasts with similar spatial frequencies are present. In general, such visual masking increases with masker contrast magnitude \cite{daly1992visible}.
Contrast perception is often modelled by a transducer function that for any input contrast magnitude provides the HVS response for such contrast \cite{foley1994human}. 
Employing contrast transducers proved beneficial in many applications including image compression \cite{daly2000visual}, image quality evaluation \cite{lubin1995visual, mantiuk2021fovvideovdp}, rendering \cite{bolin1998perceptually, ramasubramanian1999perceptually}, and foveated rendering \cite{tursun2019luminance}.

In this work, we adapt the transducer function as proposed in the context of JPEG2000 compression \cite{daly2000visual}, where a compressive power function of contrast magnitude models self-contrast masking that is further suppressed by the sum of contrast activities in the image neighborhood akin to visual masking (refer to Eq. \ref{eq:masking}).
Existing work applies contrast transducers in the primary image contrast domain (or disparity domain \cite{didyk2010apparent}), where typically image contrast is decomposed into different frequency bands using a filter bank such as Laplacian pyramid \cite{peli1990contrast, mantiuk2021fovvideovdp}, cortex transform \cite{daly1992visible}, wavelets \cite{daly2000visual}, or discrete cosine transform (DCT) \cite{watson1993visually}, and then the HVS contrast response is derived for each band.
We take an inspiration from this work, but instead of using pre-defined filter banks, we consider neural network channels, where optimal filters are learned for a task at hand. More precisely, we compute per-channel contrast signal over feature maps, apply a transducer function, and formulate a novel loss function that is aware of such feature contrast transduction. 
%Such formulated loss gives the network more freedom in changing absolute magnitude of strong features, in particular, when in the image spatial neighborhood similar features are present. 
Note that by modeling feature masking per channel, features with similar frequency characteristics act as maskers, as it is assumed in contrast visual masking.
%-------------------------------------------------------------------------
\subsection{Tone Mapping}
\subsubsection{Traditional Methods}
Traditional tone mapping methods can be roughly categorized into global methods that apply same transfer function to the whole image \cite{drago2003adaptive,jack1993tone,larson1997visibility,mantiuk2008display}, and local methods that consider the influence of neighborhood pixels \cite{fattal2002gradient,reinhard2002photographic,durand2002fast,mantiuk2006perceptual}. 
An interested reader may rafer to extensive surveys that in length discuss such methods \cite{reinhard2010high,banterle2017advanced,mantiuk2015ency}.
Recently, other model-based algorithms have been proposed, which demonstrate further performance improvement, and we include them to our comparisons in Sec.~\ref{objective comparisons} and briefly characterize here. Shan et al. \cite{shan2009globally} adopt the sliding window with optimization to keep the details. Liang et al. \cite{liang2018hybrid} design a hybrid $l_{1}$-$l_{0}$ edge-preserving filter in HSV color space to obtain more visual pleasing results. Li et al. \cite{li2018clustering} control the local weights through clustering.
Overall the traditional methods are model-based, need to introduce prior information, and the parameter-setting is not user-friendly for the non-expert users.
The closest to our goals are gradient domain techniques \cite{mantiuk2006perceptual,fattal2002gradient,shibata2016gradient} that effectively compress/enhance contrast. Mantiuk et al. \cite{mantiuk2006perceptual} drives such contrast processing by a perceptual self-contrast masking model as proposed in \cite{kingdom1996contrast}.   The key difference is that they perform processing in image contrast domain, while we consider instead feature contrast.
In exposure fusion, an HDR input image is not required and tone mapped image is merged directly from differently exposed LDR input images. Mertens et al. \cite{mertens2007exposure} select the valid regions in the input images based on contrast, saturation and well-exposedness, and then fuse them to get the final image. In our network we employ image fusion in the feature space where it is fully learned and driven by our feature contrast masking loss.



\subsubsection{Learning-based Methods}
Currently, deep learning is widely used in image processing fields, and an increasing number of learning-based tone mapping is proposed. Hou et al. \cite{hou2017deep} put forward a tone mapping method that is optimized via VGG \cite{johnson2016perceptual}. Patel et al. \cite{patel2017generative} first apply the adversarial network to tone mapping to keep the naturalness. Yang et al. \cite{yang2018image} propose a network that can simultaneously complete inverse tone mapping and tone mapping. Zhang et al. \cite{zhang2019deep} implement tone mapping in HSV color space and design different subnetworks for each component. Rana et al. \cite{rana2019deep} adopt the conditional generation adversarial network (c-GAN) for tone mapping and use multi-scale generators and discriminators to optimize the network from multi-scale. Su et al. \cite{su2021explorable} propose an explorable tone mapping network based on BicycleGAN \cite{zhu2017multimodal}, which can control the results through latent code. Most of these learning methods are fully supervised, which need paired training data. A common way to generate the dataset is that selecting the best result from a pool of tone-mapped images according to the TMQI \cite{yeganeh2012objective} score or manually. Panetta et al. \cite{panetta2021tmo} design a parameter-free tone mapping network with a generative adversarial network.  Zhang et al. \cite{9454333} make use of cycle GAN to design a semi-supervised tone mapping network, which tries to alleviate the dataset limitation. Guo et al. \cite{guo2021deep} introduce image quality assessments as a semi-supervised loss function to train a multi-scale tone mapping network. Actually, there is no perfect tone mapping operator, so the label is not reliable. In addition, the tone mapping outcome is restricted by the characteristics of images seen in the training and used there tone mapping methods. Our method is label-free, and can freely explore any HDR content as we always transform the input HDR image to make it network friendly, and through our loss that directly refers to such input we have a strickter control over the appearance of tone mapped image, and thus we leave less room for unexpected network behavior. 
%-------------------------------------------------------------------------
%Reinhard et al. \cite{reinhard2002photographic} propose an adaptive parameter Gaussian filter to acquire the details. Durand et al. \cite{durand2002fast} use the bilateral filter to extract the base layer of the HDR images.

%-------------------------------------------------------------------------

\section{Proposed Method}
\label{proposed methods}
In this section, we will illustrate our algorithm in detail, the multiple exposure fusion inputs, adaptive $\mu$-law, and feature contrast maskingl loss. The overview structure is shown in Fig.\ref{fig:pipeline}. The HDRI input is exposure-sampled into different exposed LDR images, which contain the information of all exposure intervals. The three images are taken into the same encoder via weights sharing and fused by the feature fusion module, then transformed to image form feature space through the decoder. Adaptive $\mu$-law is applied to the HDR images in order to adjust the brightness and global contrast, and feature contrast masking loss can control the local contrast.

\begin{figure*}[tbp]
\centering
\includegraphics[width=\linewidth]{./figures/pipeline.pdf}
\hfill
\caption{\label{fig:pipeline}%
The overview structure of our method. The HDRI is first exposure-sampled to generate three different exposed-LDRI, then the LDRIs are taken into the encoder to be extracted the high dimensional feature. After fusing by the fusion module, the features are transformed back into images space via the decoder. The adaptive $\mu$-lawed HDRI is served as the guidance, and visual-masked perceptual loss is the loss function for optimization. The encoder is consists of three convolution layers, the kernel size is 3 $\times$ 3, channels are 16, 32, 64 with stride 1. The fusion module is consists of 2 convolution layers, channels are both 192 with stride 1. The decoder is consists of three convolution layers, the channels are 32, 16, 3 with stride 1.  Relu \cite{nair2010rectified} is taken as the activation function, except the last decoder layer using sigmoid \cite{narayan1997generalized} to map the output in the range [0, 1].  For more stable training and faster convergence,  a residual connection is added between input and output.
}
\end{figure*}


%-------------------------------------------------------------------------
\subsection{Multiple Exposure Fusion Pipeline}
\label{mef}
HDR images are linear storage and have an extremely large dynamic range compared with LDR images, moreover, the distribution of pixel intensity in the HDR image is also unbalanced, where most pixels are concentrated on the low intensity. The linear storage and unbalanced distribution will make it harder for the network to converge, and general practice is using the logarithm of HDR as input \cite{zhang2019deep, su2021explorable}. However, during our experiments, we find the logarithm method will lead to the tone mapping results unnatural brightness, see Section \ref{ablation studies}. 
%Inspired by the generation of HDR radiance map \cite{debevec2008recovering}, which utilizes multiple exposures LDR images to generate one HDR image, we design an inverse pipeline of it. Specifically, we first sample the exposure of the input HDR to obtain multiple exposure LDR sequences, and fuse them in feature space through a convolution network, then decode back to get the final tone mapping result. According to this operation, we transfer the directly HDR image compression into LDR images information fusion, which can generate more natural results. Fig. \ref{fig: mef} shows the details.
%\begin{figure}[tbp]
%\centering
%\includegraphics[scale = 0.6]{./figures/mef.pdf}
%\includegraphics[scale = 0.6]{./figures/mes.pdf}
%\hfill
%\caption{\label{fig: mef}%
%Examples of HDR generation and exposure sampling. The top row is the HDRI generation pipeline, multiple exposed LDRIs are fused to generate the HDRI. The bottom row is the exposure sampling pipeline, the HDRI is exposure-sampled into multiple exposed LDRIs, the HDRI's information can be preserved in these LDRIs.
%}
%\end{figure}
%\subsubsection{Exposure Sampling}
%\label{ep}
Because most of the HDR images are stored as relative values, before sampling the HDRI, we first need to normalize the HDRI's mean to 0.5. Afterwards, we apply sigmoid function to lead into non-linearity to generate multiple exposure LDRIs. 
\begin{align}
I_{e} &= (1+s)\frac{ H_{e}^{n} }{H_{e}^{n}  +  s} \\
H_{e} &= \mathrm{clip}(2^{e/2}\cdot H)
\end{align}
H is the original HDR image. $H_{e}$ represents the sampled HDRI, $e$ is the exposure factor, clip($\ast$) is a function to clip the intensity into [0, 1], and $I_{e}$ is the generated LDRI. Equation (1)  is a sigmoid function to introduce the non-linearity, in this paper, $s = 0.6$,  $n = 0.9$. 
%$(1 + a)\frac{ H_{e_{i}}^{n}}{ H_{e_{i}}^{n} + a}$  is a sigmoid function to introduce the non-linearity, here, a = 0.6,  n = 0.9. 

The most significant thing of exposure sampling is determining the exposure factor $e$. We take use of \cite{andersson2021visualizing} to calculate the start and stop exposure factor, w.r.t $e_{start}$ and $e_{stop}$. After experiments, we find that three different exposures are proper, less exposures will lead to information missing to make results worse and more will lead to information redundancy with more computational consumption. The selected exposure factors are  $e_{start}$, $e_{stop}$, and $(e_{start} + e_{stop})/2$. 

%\subsubsection{Network Structure}
%\label{network structure}
Our network, as shown in  Fig. \ref{fig:pipeline},  is consists of eight convolution layers. In particular, three layers for the encoder, two layers for the fusion module, and three layers for the decoder. Especially, in order to use the model efficiently, weights sharing is applied to the encoder, this is to say, different inputs will be taken into the same encoder.
%'K*K, C, S' represents, the convolution kernel size, feature channels , and convolution strides. Relu is taken as activation function for enocder and decoder, expcept the last decoder layer using sigmoid to make output in range [0, 1].
%For the encoder, all of the convolution kernel sizes are 3 $\times$ 3 with stride 1, and the output channels are 16, 32, 64. The first layer kernel size of the fusion module is 3 $\times$ 3, and the second is 1 $\times$ 1. Both of the strides are 1 with output channels 192. As for the decoder, all of the kernel sizes are 3 $\times$ 3 with stride 1, and channels are 32, 16, 3.

%\begin{figure}[tbp]
%\centering
%\includegraphics[width=\linewidth]{./figures/network.pdf}
%\hfill
%\caption{\label{fig: network}%
%Translation Network architecture. The encoder is consists of three convolution layers, the kernel size is 3 $\times$ 3, channels are 16, 32, 64 with stride 1. The fusion module is consists of 2 convolution layers, channels are both 192 with stride 1. The decoder is consists of three convolution layers, the channels are 32, 16, 3 with stride 1.  Relu \cite{nair2010rectified} is taken as the activation function, except the last decoder layer using sigmoid \cite{narayan1997generalized} to map the output in the range [0, 1].  For more stable training and faster convergence,  a residual connection is added between input and output.
%}
%\end{figure}
%-------------------------------------------------------------------------
\subsection{Adaptive $\mu$-law}
\label{mu law}
Similarly, directly using the original HDR radiance map to optimize the network is inappropriate, which has an extremely wider dynamic range and is not satisfied with Human Visual Systems (HVS). Inspired by $\mu$ law, which is widely used in HDR coding \cite{jinno2011mu} and inverse tone mapping \cite{wu2018hdr, Marcel:2020:LDRHDR}, we further improve it and propose the adaptive $\mu$-law to have a better control of the contrast and brightness for the tone mapping results. Because there is a big difference between different scenarios, such as the sun in the sky and candles in the darkroom, using a fixed $\mu$ can not handle all the scenes, which will lead to over-exposed or under-exposed for the results. Since the HDR images' mean has been normalized to 0.5, the median value of the HDR images could be a good criterion for adaptive $\mu$ selection, which can be treated as the overall exposure intensity. We first calibrate some median value and $\mu$ pairs by experiments, guiding by the TMQI,  and then find these can be well-fitted by a power curve, which is shown in Fig. \ref {fig:fitted_curves}. The final adaptive $\mu$-law is as follows.

\begin{figure}[tbp]
\centering
\includegraphics[width=0.8\linewidth]{./figures/fitted_curve.pdf}
\hfill
\caption{\label{fig:fitted_curves}%
The fitted curves of median value adaptive $\mu$. The horizontal axis is the median value, and the vertical axis is the $\mu$. For better visualization, the vertical axis is represented in logarithmic space.
}
\end{figure}
%We select the paprmeter $\mu$ adaptively based on the median value of HDR images.
%After experiments, we fine tune the interval and $\mu$, the final equation is,
%First, we use K-means to coarsely cluster the HDR median values, and choose proper $\mu$ based on the median value. After experiments, we fine tune the interval and $\mu$, the final equation is,
%\begin{equation}
%H_{\mu} = \frac{log(1 + \mu \ast H)}{log(1 + \mu)}
%\left\{
%\begin{array}{lr}
%\mu = 4.0, &  H_{med} \geq 0.2 \\
%\mu = 10.0, &  0.2 > H_{med} \geq 0.1 \\
%\mu = 100.0, & 0.1 > H_{med} \geq 0.02 \\
%\mu = 5000.0, &  otherwise\\
%\end{array}
%\right.
%\end{equation}
\begin{equation}
H_{\mu} = \frac{\mathrm{log}(1 + \mu \cdot H)}{ \mathrm{log}(1 + \mu)}
\end{equation}
\begin{equation}
\mu = a \cdot V_{median}^{b}  + c \cdot V_{median}^{d}
\end{equation}
$H_{\mu}$ is the compressed HDR, and $V_{median}$ is the median value of the HDR image. Here, $a = 8.759$, $b = 2.148$, $c = 0.1494$, $d = -2.067$. Generally, the median value can represent the brightness of the HDR images, in that case, more compression can be applied to the dark image, and less to the brighter one. Fig. \ref{fig:mu-law} shows an example of adaptive $\mu$-law, we can see the distribution of the original HDR radiance map is unbalanced, a lot of pixels are concentrated in low intensity, and the dynamic range is extremely large, which is the obstacle for the network to learn useful information. Applying the adaptive $\mu$-law can compress the dynamic range, and make the distribution more balanced, see Fig. \ref{fig:mu-law}. On the other hand, since we adopt VGG \cite{simonyan2014very} as the perceptual loss, the $\mu$-lawed HDRI has more similar range to the original input.
% \begin{figure}[tbp]
%\centering
%\includegraphics[width=\linewidth]{./figures/mu_law.pdf}
%\hfill
%\caption{\label{fig:mu-law}%
%Example of adaptive $\mu$-law. The top right is the histogram of the HDR image, shown in left, and the bottom is the histogram after applying apdative $\mu$-law, which compress the global contrast and make it easier for network to learn. 
%}
%\end{figure}
 \begin{figure}[tbp]
\centering
\includegraphics[width=\linewidth]{./figures/mu_law_hist.pdf}
\hfill
\caption{\label{fig:mu-law}%
Example of adaptive $\mu$-law. The top row is the original HDRI with its histogram, and the bottom is the adaptive $\mu$-lawed HDR image with its histogram. We can see the distribution of histograms becomes more balanced, which will make it easier for the network to learn the information. It should be noted that for better visualization, the vertical axis of the original HDRI's histogram is represented in logarithm space.
}
\end{figure}



%-------------------------------------------------------------------------
\subsection{Feature Contrast Masking Loss}
\label{vml}

In this section, we elaborate in detail on how to optimize the network with our feature contrast masking loss. As described in the previous section, we use the adaptive $\mu$-lawed HDRI as the label, we select perceptual loss \cite{johnson2016perceptual} as the basic loss function rather than $L_{1}$ loss, the comparisons between these two loss are shown in sec \ref{loss comparisons}. However, during the experiments, we find the adaptive $\mu$-law does well in global contrast and brightness for the tone mapping results while fail in maintaining and adjusting local contrast consistency between tone mapped image and the original HDRI, which is critical in tone mapping. Therefore, inspired by the visual masking model, we design a novel feature contrast masking loss to handle the issue. The traditional visual masking model is applied to the image space, which can suppress high-contrast areas and enhance low-contrast parts. On the basis of this, we further propose a visual masking model in feature space, which can be proved by experiments that have a better local contrast control than implementing in image space, in addition, implementing on images can also lead to brightness distortion, see the results in section \ref{fai}.
The model formulation is as follows:
\begin{equation}
\hat{F}(i, j) =\frac{\mathrm{sign}(\frac{F(i, j) - {\mu}_{g}(i, j)}{{\mu}_{g}(i,  j)})^{\gamma}}{{C + \mathrm{sign}(\frac{{\sigma}_{b}(i, j)}{{\mu}_{b}(i, j)})}^{\beta}}
\label{eq:masking}
\end{equation}
\begin{equation}
{\mu}_{g}(i, j) = \sum\limits_{k = -K}^{K}\sum\limits_{l = -L}^{L}\omega_{{g}_{k,  l}}F_{k, l}(i, j)
\end{equation}
\begin{equation}
{\mu}_{b}(i, j) = \sum\limits_{p = -P}^{P}\sum\limits_{q = -Q}^{Q}\omega_{{b}_{p,  q}}F_{p, q}(i, j)
\end{equation}
\begin{equation}
\sigma_{b}(i, j) = \sqrt{ \sum\limits_{p = -P}^{P}\sum\limits_{q = -Q}^{Q}(\omega_{{b}_{p,  q}}(F_{p, q}(i, j) - {\mu}_{b}(i, j))^{2})}
\end{equation}
$F(i, j)$ is the original feature map, and $\hat{F}(i, j)$ is the processed feature map. $i = 1, 2$, $\cdots$, $M, j = 1, 2$, $\cdots$, $N$ are spatial indices, M and N are the height and width of the feature map. $C = 1$ is constant to avoid the denominator tending to zero, e.g., the flat regions. The numerator is the normalized difference of the original feature and local mean ${\mu}_{g}(i, j)$, which will enhance the local contrast. The denominator is normalized local standard deviation, which can suppress the large contrast region. ${\mu}_{g}(i, j)$ is calculated by Gaussian filter. ${\mu}_{b}(i, j) $ and $\sigma_{b}(i, j)$ is calculated by box filter. $K$, $L$ are the kernel size of the Gaussian filter, and $P$, $Q$ are of the box filter. We select $K = L =6$, and $P = Q = 6$ in this paper. The whole feature contrast maskingl can control the local contrast through $\beta$ and $\gamma$. Finally, the feature contrast masking loss can be expressed as:
\begin{equation}
L = \frac{1}{C_{m}H_{m}W_{m}} \left |\left|  \hat{F}_{m}(I_{hdr}) - \hat{F}_{m}(I_{ouput})\right | \right|_{1}
\end{equation}
$\hat{F}_{m}$ represents the \textit{m}th layer feature map applying visual masking model, $C_{m} \times H_{m} \times W_{m}$ is the shape. The feature contrast masking loss is $L_{1}$ norm between the feature maps. It is worth noting that in order to have good control of the local contrast, we keep the $\gamma$ and $\beta$ of the output masking is 1, and only adjust them of  HDRI masking. At last, we apply gamma correction for the outputs \cite{schlick1995quantization, banterle2017advanced, qiu2007learning} for color correction. 
\begin{figure*}[tbp]
\centering
\includegraphics[width=\linewidth]{./figures/vis_masking.pdf}
\hfill
\caption{\label{fig: vis_masking}%
Visualization of the 2nd layer 100th channel of VGG19, from the left to right is the input contrast pattern, the original feature map, the visual masked feature map, the numerator and denominator of the visual masking model. Here, we choose gamma and beta both are 0.5.
}
\end{figure*}
Fig. \ref{fig: vis_masking} shows a visualization of the feature contrast masking. The input is a test image from \cite{wolski2018dataset}, which contains various contrast patterns. From the visualization, we can see, after using feature contrast masking, more local contrast appears, the numerator can emphasize the local contrast, and the denominator has a strong response in the high contrast region, weak in low contrast regions, which means it can suppress high contrast and boost low contrast.

%See Section \ref{non-lin} and \ref{loss comparisons} for further exploration of why using perceptual loss, why apply visual masking in feature maps rather than images, and how visual masking control the local contrast.
%-------------------------------------------------------------------------
\section{Results and Ablation Study}
\label{experiment}
In this section, we will elaborate in detail on the implementation, the objective and subjective comparisons, and ablation study.
%------------------------------------------------------------------------
\subsection{Implementation}
\label{implementation}
We adopt an online training strategy, this is to say, we train a model for each HDR image at test time. On one hand, we do not need external labels, online training is suitable. On the other hand, it only takes several minutes for training rather than several days as offline training. In detail, our model is implemented on the deep learning platform TensorFlow with GPU RTX 8000. The network is optimized by Adam with an initial learning rate $10^{-4}$.

%------------------------------------------------------------------------
\subsection{Objective Comparisons}
\label{objective comparisons}

We adopt the TMQI \cite{yeganeh2012objective}, BTMQI\cite{gu2016blind}, and BRISQUE \cite{mittal2012no} as the metrics. The former two metrics are widely used in tone mapping evaluation \cite{guo2021deep, 9454333, liang2018hybrid}, and BRISQUE is a good blind metric to evaluate the contrast distortion \cite{jiang2019nighttime, lim2017contrast, song2020enhancement}. 180 test images are selected, 93 from Fairchild \cite{fairchild2007hdr}, 42 from HDRIheaven $\footnote{\url{https://polyhaven.com/hdris}}$, and 45 from Laval HDRI \cite{gardner2017learning}, which cover various scenes, indoors, outdoors, brighter and darker scenes.

TMQI is a full-reference tone mapping image quality assessment, which is consists of structural fidelity and naturalness. The structural fidelity is modified based on SSIM \cite{wang2004image}, which mainly measures the difference of structure between tone mapping images and the reference HDR images. The naturalness is highly related to brightness and contrast, which can evaluate how natural the images look. $\mathrm{TMQI_{S}}$ expresses structural fidelity and $\mathrm{TMQI_{N}}$ represents the naturalness, and TMQI score is a combination of them. It is worth noting that structural fidelity has a higher weight in the original implementation. A larger TMQI score means a better result.

%which can be modeled with the mean and standard deviation of the images and fitted by Gaussian and Beta probability density functions

BTMQI is a no-reference tone mapping metric, which is composed of three terms. The first term calculates the global and local entropy that can gauge the information contained in the image, which can measure the richness of information. The second term is the same as the naturalness in TMQI. The third measures the image structural information via computing the intensity of the Sobel-filtered image. Finally, these three terms will be regressed with SVR to get the final score. A lower BTMQI represents better performance.

BRISQUE is a well-known no-reference image quality assessment, which mainly gauges the naturalness of images. It first extracts the mean subtracted contrast normalized (MSCN) coefficients from the image, which is a good feature to evaluate the distortion. In addition, it also builds the neighborhood relationships by MSCN coefficients. At last, applying the SVR to these features to compute the final score. A lower BRISQUE score is desired.

Overall, TMQI and BTMQI mainly consider the naturalness and structure fidelity. Good structure fidelity means, the tone mapping image has a closer structure to the HDR image and good naturalness represents tone mapping images is more comparable with the natural LDR image, especially for the brightness and contrast. They have a similar measurement for naturalness while different assessments for structure fidelity, one is a full reference and another is no reference. BRISQUE is mainly for the contrast distortion. In addition, TMQI focus on the global contrast while BRISQUE pay more attetion to the local contrast.  

Eleven other tone mapping operators are selected as the comparison methods, for simplicity, which can be expressed as Guo \cite{guo2021deep}, Zhang \cite{9454333}, Yang \cite{yang2018image}, Liang \cite{liang2018hybrid}, Shibata \cite{shibata2016gradient}, Li \cite{li2018clustering}, Shan \cite{shan2009globally}, Durand \cite{durand2002fast}, Drago \cite{drago2003adaptive}, Mertens \cite{mertens2007exposure}, Ramman \cite{raman2009bilateral}, and Reinhard \cite{reinhard2002photographic}. The first three are learning-based methods and others are traditional methods. Guo \cite{guo2021deep}, Zhang \cite{9454333}, Yang \cite{yang2018image}, Liang \cite{liang2018hybrid}, Shibata \cite{shibata2016gradient}, Li \cite{li2018clustering}, and Shan \cite{shan2009globally} are tested with their publish codes and Durand \cite{durand2002fast}, Drago \cite{drago2003adaptive}, Mertens \cite{mertens2007exposure}, and Reinhard \cite{reinhard2002photographic} are implemented with HDRToolBox \cite{banterle2017advanced}.
Here, we set the gaussian kernel size is 13 $\times$ 13, $\gamma$ is 0.5, and $\beta$ is 0.5. The testing results are shown in Table \ref{tabel: evaluation results}.
\begin{table*}
 	\caption{\label{tabel: evaluation results}%
           Comparison with other methods. Mean and standard deviation for 180 test images form three different dataset.
           }
	\centering
	 \begin{tabular}{|c | c | c | c | c | c | } 
	 \hline
	 Methods & TMQI ($\uparrow$) &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$)  & BTMQI ($\downarrow$) & BRISQUE ($\downarrow$)\\ [0.5ex] 
	 \hline
	 Ours & \textbf{0.9250 $\pm$ 0.0438} &\textbf{0.8891 $\pm$ 0.0579} &  \textbf{0.7040 $\pm$ 0.2379} & \textbf{3.0075 $\pm$ 1.003} & \textbf{20.7904 $\pm$ 8.3566} \\ 
	 \hline
            Guo \cite{guo2021deep} & 0.8814 $\pm$ 0.0364  & 0.8124 $\pm$ 0.0799 & 0.5664 $\pm$ 0.2135 &3.9474 $\pm$ 1.0201  &  24.7113 $\pm$ 8.5391 \\         
           \hline
	 Zhang \cite{9454333} & 0.8861 $\pm$ 0.0412 &0.8246 $\pm$ 0.0925 & 0.5821 $\pm$  0.2724 & 3.4532 $\pm$ 1.3503 & 23.4535 $\pm$ 9.4469 \\ 
	 \hline
	 Yang \cite{yang2018image} & 0.8316 $\pm$ 0.0779 & 0.7658 $\pm$ 0.1196 &  0.3973 $\pm$ 0.2921 & 4.4123 $\pm$ 1.4601 & 39.4103 $\pm$ 8.8768 \\ 
	 \hline
	 Liang \cite{liang2018hybrid} & 0.8920 $\pm$ 0.0498 &0.8545 $\pm$  0.0710 & 0.5639 $\pm$ 0.2627 & 3.7766 $\pm$ 1.0834  & 25.6813 $\pm$ 8.8136 \\
	 \hline
	 Shibata \cite{shibata2016gradient} & 0.7555 $\pm$ 0.0462 &0.7241 $\pm$ 0.08841 &  0.0992 $\pm$ 0.1541 & 4.4472 $\pm$ 0.7880 & 31.3008 $\pm$ 9.6664\\
	 \hline
	 Li \cite{li2018clustering} & 0.8303 $\pm$ 0.0557 &0.8230 $\pm$ 0.0751 & 0.2914 $\pm$ 0.2698 & 4.7775 $\pm$ 0.9990 & 23.0962 $\pm$ 8.0272\\
	 \hline
	 Shan \cite{shan2009globally} &  0.8250 $\pm$ 0.0736  & 0.7431 $\pm$ 0.1528 & 0.3946 $\pm$ 0.2696 & 4.2162 $\pm$ 0.9684  & 24.0481 $\pm$ 9.0589\\ 
	\hline
	Durand \cite{durand2002fast} & 0.8595 $\pm$ 0.0738 &0.8219 $\pm$ 0.1064 & 0.4427 $\pm$ 0.2853 & 3.8821 $\pm$ 1.1785 & 21.8206 $\pm$ 8.6475\\
	\hline
	Drago \cite{drago2003adaptive} & 0.8855 $\pm$0.0525 & 0.8676 $\pm$0.0727  & 0.5077 $\pm$ 0.2668 & 3.8372 $\pm$ 1.2828 &  22.9493 $\pm$  9.0658\\
	\hline
	Mertens \cite{mertens2007exposure} & 0.8431 $\pm$ 0.0771 &0.8457 $\pm$ 0.0909 & 0.3373 $\pm$  0.2958 & 4.4434 $\pm$ 1.6311 & 23.3920 $\pm$ 9.6142\\
	\hline
%	Ramman\cite{raman2009bilateral}  & 0.8191 $\pm$ 0.0864 & 0.8302 $\pm$ 0.1207 &0.2534 $\pm$  0.2862 & 5.0304 $\pm$ 1.5265 &25.1065  $\pm$ 10.0342\\
%	\hline
	Reinhard \cite{reinhard2002photographic} &0.8530 $\pm$ 0.0545 & 0.8224$\pm$ 0.0837  & 0.3950  $\pm$ 0.2328 & 4.1901 $\pm$ 1.4792 & 25.6866 $\pm$  8.1615\\ [1ex] 
	 \hline
	\end{tabular}
\end{table*}

%\begin{table*}
% 	\caption{\label{tabel: evaluation results}%
%           COMPARISON WITH OTHER METHODS
%           }
%	\centering
%	 \begin{tabular}{|c | c | c | c | c | c | } 
%	 \hline
%	 Methods & $TMQI_{Q}$ ($\uparrow$) &$TMQI_{S}$ ($\uparrow$) & $TMQI_{N}$ ($\uparrow$)  & BTMQI ($\downarrow$) & BRISQUE ($\downarrow$)\\ [0.5ex] 
%	 \hline
%	 Ours & \textbf{0.9251} &\textbf{0.8891}  & \textbf{0.7041}   & \textbf{3.0075}  &\textbf{20.7904} \\ 
%	 \hline 
%           Guo \cite{guo2021deep} &0.8814 & 0.8124  & 0.5664  & 3.9474 & 24.7113 \\
%           \hline
%	 TMM21 \cite{9454333} & 0.8861  &0.8246  & 0.5821 & 3.4532  & 23.4535  \\ 
%	 \hline
%	 DHRT \cite{yang2018image} & 0.8316 & 0.7658  &  0.3973  & 4.4123 & 39.4103\\ 
%	 \hline
%	 CVPR18 \cite{liang2018hybrid} & 0.8920  &0.8545  & 0.5639  & 3.7766  & 25.6813 \\
%	 \hline
%	 CVPR16 \cite{shibata2016gradient} & 0.7555  &0.7241  &  0.0992 & 4.4472 & 31.3008 \\
%	 \hline
%	 CVIU16 \cite{li2018clustering} & 0.8303  &0.8230  & 0.2914 & 4.7775  & 23.0962 \\
%	 \hline
%	 TVCG09 \cite{shan2009globally} &  0.8250  & 0.7431  & 0.3946  & 4.2162 & 24.0481\\ 
%	\hline
%	Durand \cite{durand2002fast} & 0.8595  &0.8219 & 0.4427 & 3.8821& 21.8206 \\
%	\hline
%	Drago \cite{drago2003adaptive} & 0.8855 & 0.8676  & 0.5077  & 3.8372 &  22.9493 \\
%	\hline
%	Mertens \cite{mertens2007exposure} & 0.8431  &0.8457 & 0.3373 & 4.4434 & 23.3920 \\
%	\hline
%	Ramman\cite{raman2009bilateral}  & 0.8191  & 0.8302 &0.2534  & 5.0304 &25.1065  \\
%	\hline
%	Reinhard \cite{reinhard2002photographic} &0.8530  & 0.8224  & 0.3950   & 4.1901  & 25.6866 \\
%	 \hline
%	\end{tabular}
%\end{table*}

%\begin{table*}
% 	\caption{\label{tabel: evaluation results}%
%           COMPARISON WITH OTHER METHODS
%           }
%	\centering
%	 \begin{tabular}{|c | c | c | c | c | c | } 
%	 \hline
%	 Methods & $TMQI$ ($\uparrow$) &$TMQI_{S}$ ($\uparrow$) & $TMQI_{N}$ ($\uparrow$)  & BTMQI ($\downarrow$) & BRISQUE ($\downarrow$)\\ [0.5ex] 
%	 \hline
%	 Ours & \textbf{0.9251} &\textbf{0.8891}  & \textbf{0.7041}   & \textbf{3.0075}  &\textbf{20.7904} \\ 
%	 \hline 
%           Guo \cite{guo2021deep} &0.8814 & 0.8124  & 0.5664  & 3.9474 & 24.7113 \\
%           \hline
%	 Zhang \cite{9454333} & 0.8861  &0.8246  & 0.5821 & 3.4532  & 23.4535  \\ 
%	 \hline
%	 Yang \cite{yang2018image} & 0.8316 & 0.7658  &  0.3973  & 4.4123 & 39.4103\\ 
%	 \hline
%	 Liang \cite{liang2018hybrid} & 0.8920  &0.8545  & 0.5639  & 3.7766  & 25.6813 \\
%	 \hline
%	 Shibata \cite{shibata2016gradient} & 0.7555  &0.7241  &  0.0992 & 4.4472 & 31.3008 \\
%	 \hline
%	  Li \cite{li2018clustering} & 0.8303  &0.8230  & 0.2914 & 4.7775  & 23.0962 \\
%	 \hline
%	 Shan \cite{shan2009globally} &  0.8250  & 0.7431  & 0.3946  & 4.2162 & 24.0481\\ 
%	\hline
%	Durand \cite{durand2002fast} & 0.8595  &0.8219 & 0.4427 & 3.8821 & 21.8206 \\
%	\hline
%	Drago \cite{drago2003adaptive} & 0.8855 & 0.8676  & 0.5077  & 3.8372 &  22.9493 \\
%	\hline
%	Mertens \cite{mertens2007exposure} & 0.8431  &0.8457 & 0.3373 & 4.4434 & 23.3920 \\
%	\hline
%	Reinhard \cite{reinhard2002photographic} &0.8530  & 0.8224  & 0.3950   & 4.1901  & 25.6866 \\
%	 \hline
%	\end{tabular}
%\end{table*}
From the comparison, we can find that our method outperforms others. In detail, the highest $\mathrm{TMQI_{S}}$ score means that our results are more similar to the HDR images in terms of structure. The $\mathrm{TMQI_{N}}$ score indicates that our results have a better appearance of contrast and brightness. The lowest BTMQI score reveals our results contain more information and have a more natural representation. The lowest BRISQUE score means less contrast distortion. In addition, we can find that the learning-based algorithms Guo  \cite{guo2021deep} and Zhang \cite{9454333} have a good performance in $TMQI_{N}$ while poor performance in BRISQUE, which means the results have proper brightness and global contrast with distorted local contrast. Liang \cite{liang2018hybrid} has an excellent $\mathrm{TMQI_{S}}$ and $\mathrm{TMQI_{N}}$ but doesn't work well for the BRISQUE, which means the results have unnaturalness in local contrast. The results from Yang \cite{yang2018image} and Shibata \cite{shibata2016gradient} underperform for all the metrics, which illustrates they have distortion of structural fidelity, brightness, and local and global contrast. The scores of Li \cite{li2018clustering} and Shan \cite{shan2009globally} are close and the performance is average. Li \cite{li2018clustering} woks better in structural similarity and Shan \cite{shan2009globally} is better in naturalness. Durand \cite{durand2002fast} has a lower BRISQUE score which means that the local contrast is close to the natural image. However, it doesn't work well for the $\mathrm{TMQI_{S}}$ and $\mathrm{TMQI_{N}}$, in other words, it loses the structural fidelity, brightness, and global contrast. Drago \cite{drago2003adaptive} plays excellently in $\mathrm{TMQI_{S}}$, $\mathrm{TMQI_{N}}$ and BRISQUE but slightly inferior to the BTMQI, which expresses the results lose some detail information. Mertens \cite{mertens2007exposure} and Reinhard \cite{reinhard2002photographic} are quite similar, they are good at structure-preserving but underperform in the naturalness.

which means our results have a good quality of structure maintenance, contrast fidelity, and brightness compression. This is also in line with our original design intention. 

%------------------------------------------------------------------------

\subsection{Subjective Comparisons}
\label{subjective comparisons}

We also show the visual results of our method and comparisons in Fig. \ref{fig: objective comparisons 1},  Fig. \ref{fig: objective comparisons 2} and Fig. \ref{fig: objective comparisons 3}. Since the page limitation, the eight methods with the highest TMQI score will be shown. From the images, we can see, our results are more robust for various scenes, outdoors and indoors. In particular, our results have a good quality of the global and local contrast, and will not lead to the halo, wash-out artifacts. Guo \cite{guo2021deep} can achieve good brightness and contrast while having obvious color shift. Zhang \cite{9454333} causes blurry in the results. Yang \cite{yang2018image} results artifacts in the highlight regions. Liang \cite{liang2018hybrid} performs well in terms of brightness but loses the local contrast.  Li \cite{li2018clustering} also have problems in the color preserving and contrast maintenance.  Shibata \cite{shibata2016gradient} is prone to produce images with over-exaggerated local contrast. The results of Shan \cite{shan2009globally} tends to be over-enhanced of brightness and misses details. Durand \cite{durand2002fast} leads to holo in the high contrast regions, such as the surrounding of lights. Drago \cite{drago2003adaptive} works well in the brightness but also has local contrast distortion. Mertens \cite{mertens2007exposure} produces over dark images. Reinhard \cite{reinhard2002photographic} can not handle the high contrast scenes such as the second row in Fig. \ref{fig: objective comparisons 2}. Please refer to the supplementary materials for more complete results.
%CVPR 18 is good at maintaining the local inforamtion but the results appear darker. CVPR16 will over-enhance the details, which is not natrual. CVIU16 will lead to wash-out, which is undesired in tone mapping. The overral lumiance of TVCG09 is deuced enhanced. Durand results can introduce holo artifacts. Drago and mertens will lose some local contrast. The results of Ramman and Reinhard are too dark.

%\begin{figure*}[htbp]
%\centering
%\subfigure[pic1.]{
%\begin{minipage}[t]{0.25\linewidth}
%\centering
%\includegraphics[width=1.725in]{./figures/results/ours/hdr_3.png}
%%\caption{fig1}
%\end{minipage}%
%}%
%\subfigure[pic2.]{
%\begin{minipage}[t]{0.25\linewidth}
%\centering
%\includegraphics[width=1.725in]{./figures/results/cviu16/hdr_3.png}
%%\caption{fig2}
%\end{minipage}%
%}%
%\subfigure[pic3.]{
%\begin{minipage}[t]{0.25\linewidth}
%\centering
%\includegraphics[width=1.725in]{./figures/results/cvpr18/hdr_3.png}
%%\caption{fig2}
%\end{minipage}
%}%
%\subfigure[pic4.]{
%\begin{minipage}[t]{0.25\linewidth}
%\centering
%\includegraphics[width=1.725in]{./figures/results/tvcg09/hdr_3.png}
%%\caption{fig2}
%\end{minipage}
%}%
%\centering
%\caption{ pics}
%\end{figure*}
%

%	\begin{figure*}[htb]
%	\captionsetup[subfigure]{labelformat=empty}
%		\subfloat[Ours: \textbf{0.9413}]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[TMM21: 0.8206]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[DHRT: 0.8286]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/dhrt/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[CVPR18: 0.8373]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	          \quad
%		\subfloat[CVPR16: 0.7155]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr16/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[CVIU16: 0.8626]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cviu16/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	           %\quad
%		\subfloat[TVCG09: 0.8241]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Durand: 0.7739]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/durand/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	          \quad
%		\subfloat[Drago: 0.8969]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Mertens: 0.7703]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	          %\quad
%		\subfloat[Ramman: 0.7475]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/ramman/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Reinhard: 0.8336]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_3.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\centering
%	          \quad
%		\subfloat[Ours: \textbf{0.9256}]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[TMM21: 0.8430]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[DHRT: 0.7636]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/dhrt/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[CVPR18: 0.8765]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	          \quad
%		\subfloat[CVPR16: 0.7555]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr16/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[CVIU16: 0.7360]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/cviu16/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	           %\quad
%		\subfloat[TVCG09: 0.9090]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Durand: 0.8075]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/durand/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	           \quad
%		\subfloat[Drago: 0.7896]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Mertens: 0.8655]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Ramman: 0.8191]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/ramman/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%		\subfloat[Reinhard: 0.8775]{
%			\begin{minipage}{0.225\linewidth}
%				\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_26.png}
%			\end{minipage}
%		}\hspace{-1pt}
%	
%		\centering
%	
%		\caption{\label{fig: objective comparisons}%
%	            Visual comparisons of different TM methods on testset. }
%		\label{fig:syn}
%	\end{figure*}


%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[Ours: \textbf{0.9413}]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_3_border.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Guo: 0.9013]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_3.jpg}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Drago: 0.8969]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Li: 0.8626]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cviu16/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Liang: 0.8373]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Reinhard: 0.8336]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Yang: 0.8286]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/dhrt/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Shan: 0.8241]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Ours: \textbf{0.9565}]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_137_border.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Zhang: 0.9435]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Guo: 0.9091]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_137.jpg}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Liang: 0.9073]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Drago: 0.9017]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Mertens: 0.8696]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Reinhard: 0.8518]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Shan: 0.8098]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_137.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: objective comparisons}%
%            Visual comparisons of different TM methods on testset. }
%\end{figure*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Ours: \textbf{0.9413}]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_3_border.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Guo: 0.9013]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_3.jpg}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Drago: 0.8969]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Li: 0.8626]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cviu16/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
          \quad
	\subfloat[Liang: 0.8373]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Reinhard: 0.8336]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Yang: 0.8286]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/dhrt/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Shan: 0.8241]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: objective comparisons 1}%
             Visual comparisons of different TM methods on the test set. Our result has better brightness and contrast. Guo \cite{guo2021deep} has artifacts in the highlight regions, such as the window. Drago \cite{drago2003adaptive} is good at brightness but loses local contrast, such as the floor. Li \cite{li2018clustering} also has issues with the brightness, the black regions are over-enhanced. Liang \cite{liang2018hybrid},  Reinhard \cite{reinhard2002photographic} and Yang \cite{yang2018image} are too darker. Shan \cite{shan2009globally} is over-exposed and loses local contrast.}
\end{figure*}
          
\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Ours: \textbf{0.9565}]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_137_border.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Zhang: 0.9435]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Guo: 0.9091]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_137.jpg}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Liang: 0.9073]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
          \quad
	\subfloat[Drago: 0.9017]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Mertens: 0.8696]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Reinhard: 0.8518]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Shan: 0.8098]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_137.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: objective comparisons 2}%
            Visual comparisons of different TM methods on the test set. Our result has more natural brightness and contains contrast fidelity. Zhang \cite{9454333} is good at brightness but loses local contrast, such as the clouds. Guo \cite{guo2021deep} also loses the local contrast and leads to color distortion for the grass. Liang \cite{liang2018hybrid} leads to the contrast distortion, the grass has the same brightness as the sky, which should be darker than the sky. Drago \cite{drago2003adaptive} loses the local contrast, seems to be too blurry. Mertens \cite{mertens2007exposure} loses the global contrast, so it seems to be washed out. Reinhard \cite{reinhard2002photographic} is too dark.  Shan \cite{shan2009globally} is over-exposed and loses local contrast.}
\end{figure*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Ours: \textbf{0.9676}]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_53_border.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Reinhard: 0.9208]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Guo: 0.9161]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_53.jpg}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Liang: 0.9158]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
          \quad
	\subfloat[Shan: 0.8841]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Durand: 0.8704]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/durand/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Zhang: 0.8788]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Mertnes: 0.8602]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: objective comparisons 3}%
            Visual comparisons of different TM methods on the test set. Our result is more natural and better reproduction. Reinhard \cite{reinhard2002photographic} has issue with the brightness. Guo \cite{guo2021deep} has color distortion in the grass. Liang \cite{liang2018hybrid} loses local contrast in the sky. Shang is good at brightness but loses local contrast, such as the clouds. Durand \cite{durand2002fast} is too dark. Zhang \cite{9454333} and Mertens \cite{mertens2007exposure} lose global and local contrast, so the grass seems blurry and the whole image seems washed out.}
\end{figure*}

%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[Ours: \textbf{0.9644}]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_118_border.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Drago: 0.9593]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/drago/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Durand: 0.9357]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/durand/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Liang: 0.9040]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Zhang: 0.8886]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Guo: 0.8830]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_118.jpg}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Reinhard: 0.8813]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Li: 0.8565]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cviu16/hdr_118.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Ours: \textbf{0.9676}]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/ours/hdr_53_border.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Reinhard: 0.9208]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/reinhard/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Guo: 0.9161]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/guo/hdr_53.jpg}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Liang: 0.9158]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/cvpr18/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Shan: 0.8841]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tvcg09/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Durand: 0.8704]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/durand/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Zhang: 0.8788]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/tmm21/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Mertnes: 0.8602]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/results_comparsion/mertens/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: objective comparisons 2}%
%            Visual comparisons of different TM methods on test set. }
%\end{figure*}


%------------------------------------------------------------------------

\subsection{Ablation Studies}
\label{ablation studies}

%------------------------------------------------------------------------

In this section, we will illustrate the importance of each component of our method, multiple exposure fusion pipeline (ME), adaptive $\mu$-law (Ada $\mu$-law), and feature contrast masking loss (FML). Table \ref{tabel: ablation study} demonstrates the assessment score, and it should be noted that we provide two other kinds inputs without multiple exposure, linear \cite{rana2019deep} and logarithm HDRI \cite{zhang2019deep, su2021explorable}.

We can see the complete pipeline achieve the best performance. In particular, without adaptive $\mu$-law, the $\mathrm{TMQI_{N}}$ and BTMQI has a significant drop while BRISQUE slight decline, which means it has an important improvement for brightness, since $\mathrm{TMQI_{N}}$ and BTMQI will take account into the brightness while BRISQUE mainly pays attention to the contrast. Visual masking loss plays an important role in contrast control, without visual masking, the $\mathrm{TMQI_{N}}$, BTMQI, and BRISQUE all decrease obviously, which represents contrast distortion. As for multiple exposure inputs, it has a major contribution both of contrast adjusting and brightness compression, without it, $\mathrm{TMQI_{N}}$, BTMQI, and  BRISQUE have a serve decline. What's more, the structural fidelity $\mathrm{TMQI_{S}}$ in these comparisons are approximative, and we will reveal that it mainly depends on the perceptual loss in Section \ref{loss comparisons}. In addition, the logarithm input is better than the linear one.

We also provide a visual comparison to prove each component's effect. From Fig. \ref{fig: ablation study}, we can see adaptive $\mu$-law is of importance in adjusting brightness, without it, the brightness is unnatural. Visual masking plays an important role in emphasizing the local contrast, especially for the large contrast regions, such as the cloud in the sky. And compared with multiple exposure inputs, the logarithm inputs will lead to a darker output, which means lead to brightness distortion.
%\begin{table*}
% 	\caption{\label{tabel: ablation study}%
%          ABLATION STUDY ON EACH COMPONENT.}
%	\centering
%	 \begin{tabular}{| c |c | c | c | c| c | c| c|} 
%	 \hline
%	  MEF & Adaptive $\mu$-law & VML  & TMQI ($\uparrow$) &$TMQI_{S}$ ($\uparrow$) & $TMQI_{N}$ ($\uparrow$) & BTMQI ($\downarrow$) & BRISQUE ($\downarrow$) \\ [0.5ex] 
%	\hline
%           $\checkmark$  & $\  $   & $\checkmark$  & 0.8544 $\pm$ 0.0625 & 0.8661 $\pm$ 0.1050  &0.3549 $\pm$  0.2596 & 4.3479 $\pm$ 1.4745 & 21.8619 $\pm$ 9.0248\\ 
%          \hline
%          $\checkmark$  & $\checkmark$  & $\ $  & 0.9099 $\pm$ 0.0464  &\textbf{0.8870 $\pm$  0.0653}  & 0.6067 $\pm$ 0.2399  & 3.4846 $\pm$ 1.0938 & 22.7142 $\pm$ 8.8806\\ 
%          \hline
%          $\ $ & $\checkmark$  & $\checkmark$   & 0.9005 $\pm$ 0.0430 & 0.8843 $\pm$ 0.0762 &0.5629 $\pm$  0.2341 & 3.4233 $\pm$ 0.9733 & 21.8811 $\pm$ 9.2571 \\ 
%          \hline
%          $\checkmark$ & $\checkmark$  & $\checkmark$   & \textbf{0.9220 $\pm$ 0.0412} &0.8841 $\pm$ 0.0601 &  \textbf{0.6926 $\pm$ 0.2343}   & \textbf{3.1185 $\pm$ 1.0412} &\textbf{21.0599 $\pm$ 8.5187}\\[1ex] 
%	 \hline
%	\end{tabular}
%\end{table*}

\begin{table*}
 	\caption{\label{tabel: ablation study}%
          Abalation study on each component.  Mean and standard deviation for 180 test images form three different dataset.}
	\centering
	 \begin{tabular}{| c |c | c | c | c| c | c| c|} 
	 \hline
	  ME & Ada $\mu$-law & FML  & TMQI ($\uparrow$) &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$) & BTMQI ($\downarrow$) & BRISQUE($\downarrow$) \\ [0.5ex] 
	\hline
           $\checkmark$  & $\  $   & $\checkmark$  & 0.8545 $\pm$ 0.0631  & 0.8675 $\pm$ 0.0165 &0.3543 $\pm$ 0.2573  & 4.3835 $\pm$  1.5145 & 20.8804 $\pm$ 8.8381\\ 
          \hline
          $\checkmark$  & $\checkmark$  & $\ $  & 0.9152 $\pm$ 0.0484  &\textbf{0.8926 $\pm$ 0.0628} & 0.6382 $\pm$ 0.2483 & 3.2477 $\pm$ 1.0442  & 22.1843 $\pm$ 8.7971\\ 
          \hline
	$linear$ & $\checkmark$  & $\checkmark$   & 0.8786 $\pm$ 0.1252 & 0.8205$\pm$ 0.1596 &0.6039 $\pm$  0.2957 & 3.5987 $\pm$ 1.2665 & 25.2673$\pm$ 8.8121\\ 
          \hline
          $log$ & $\checkmark$  & $\checkmark$   & 0.8806 $\pm$ 0.0427 & 0.8748 $\pm$ 0.0718 &0.45981 $\pm$  0.2039 & 3.4481 $\pm$ 0.7183 & 22.6051 $\pm$ 8.7289\\ 
          \hline
          $\checkmark$ & $\checkmark$  & $\checkmark$  & \textbf{0.9250 $\pm$ 0.0438} & 0.8891 $\pm$ 0.0579 &  \textbf{0.7040 $\pm$ 0.2379} & \textbf{3.0075 $\pm$ 1.003} & \textbf{20.7904 $\pm$ 8.3566}\\
	\hline
	\end{tabular}
\end{table*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Ours: \textbf{0.9050}]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours/hdr_136.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} feature contrast masking: 0.8790]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_masking/hdr_136.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} ME: 0.8412]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_mef/hdr_136.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} adpative $\mu$-law: 0.8427]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_mulaw/hdr_136.png}
		\end{minipage}
	}\hspace{-1pt}
          \quad
	\subfloat[Ours: \textbf{0.9230}]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours/hdr_160.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} feature contrast masking: 0.8942]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_masking/hdr_160.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} ME: 0.9105]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_mef/hdr_160.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Ours \textit{w/o} adpative $\mu$-law: 0.8181]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_no_mulaw/hdr_160.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: ablation study}%
         Visual Comparison of Ablation Study. The complete pipeline achieves the best results. Without feature contrast masking loss, the local contrast will be lost. Without multiple exposure inputs, the brightness will be darker. Without the adaptive $\mu$ law, the brightness also suffers losses. (Here, the results without multiple exposure inputs adapt the logarithmic inputs.)}
\end{figure*}

%------------------------------------------------------------------------


\section{Explorations}
\label{explorations}
%------------------------------------------------------------------------
\subsection{Exploration of Gaussian Kernel Size}
We provide the explorations of Gaussian kernel size to figure out how the kernel size influences the results. Fig. \ref{fig: different kernels} shows the visualizations, we can find that small kernels will lead to local contrast loss. The shadow of the tree are over-enhanced, which should be darker like the real scene. Too large kernel will introduce  more computations. We choose a medium size kernel, 13$\times$13.

over enhance the detail and lead to holo artifacts while large kernels will lose some local contrast and introduce more computational cost. Medium kernel size is more suitable, in our paper, we select kernel size 13 $\times$ 13.
%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[ kernel size = 3]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_61_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[kernel size = 13]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_61_13.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[kernel size = 23]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_61_23.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[kernel size = 33]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_61_33.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: different kernels}%
%           Visual explorations of different gaussian kernel size. With the kernel size increasing, the results tends to be more blurry.}
%\end{figure*}
\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[ kernel size = 3]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_3.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[kernel size = 13]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_13.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[kernel size = 33]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_31.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: different kernels}%
           Visual explorations of different gaussian kernel size. The small kernel cannot capture enough local information, and leads to local contrast loss. Too large kernel will introduce extensive calculations. We choose a medium size kernel, 13$\times$13.}
\end{figure*}
%------------------------------------------------------------------------
\subsection{Exploration of Non-linearity}
\label{non-lin}
 
We also explore the influence of non-linear parameters $\gamma$ and $\beta$ as mention in Section \ref{vml}. From Fig. \ref{fig: different weights}, we can see that the $\gamma$ and $\beta$ coordinate with each other to control the local contrast. $\gamma$ controls the non-linearity of the numerator, which can emphasize the local contrast, with $\gamma$ decreasing, more details will appear. $\beta$ can adjust the non-linearity of the denominator, which can suppress large contrast regions. For better visual pleasing results, we choose $\gamma$ = 0.5 and $\beta$ = 0.5.

%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[ $\gamma$ = 1.0, $\beta$ = 1.0]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_10_10.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 1.0, $\beta$ = 0.8]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_10_08.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 1.0, $\beta$ = 0.5]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_10_05.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 1.0, $\beta$ = 0.2]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_10_02.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[ $\gamma$ = 0.8, $\beta$ = 1.0]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_08_10.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.8, $\beta$ = 0.8]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_08_08.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.8, $\beta$ = 0.5]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_08_05.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.8, $\beta$ = 0.2]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_08_02.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.5, $\beta$ = 1.0]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_05_10.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.8]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_05_08.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[ $\gamma$ = 0.5, $\beta$ = 0.5]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_05_05.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.2]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_05_02.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.2, $\beta$ = 1.0]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_02_10.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.2, $\beta$ = 0.8]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_02_08.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.2, $\beta$ = 0.5]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_02_05.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.2, $\beta$ = 0.2]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_61_02_02.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: different weights}%
%           Visual explorations of different weights of $\gamma$ and $\beta$.  $\gamma$ controls the non-linearity of the numerator, which can emphasize the local contrast, with $\gamma$ decreasing, more details will appear. $\beta$ can adjust the non-linearity of the denominator, which can suppress large contrast regions.}
%\end{figure*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[ $\gamma$ = 0.9, $\beta$ = 0.9]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.9.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$\gamma$ = 0.9, $\beta$ = 0.5]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.5.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$\gamma$ = 0.9, $\beta$ = 0.1]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.1.png}
		\end{minipage}
	}\hspace{-1pt}
           \quad
	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.9]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.9.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[ $\gamma$ = 0.5, $\beta$ = 0.5]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.5.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.1]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.1.png}
		\end{minipage}
	}\hspace{-1pt}
           \quad
	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.9]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.9.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.5]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.5.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.1]{
		\begin{minipage}{0.3\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.1.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: different weights}%
           Visual explorations of different weights of $\gamma$ and $\beta$.  $\gamma$ controls the non-linearity of the numerator, which can emphasize the local contrast, with $\gamma$ decreasing, more details will appear, as each column shows. $\beta$ can adjust the non-linearity of the denominator, which can suppress large contrast regions, as each row shows. $\gamma$ and $\beta$ cooperate to control the contrast.}
\end{figure*}



%------------------------------------------------------------------------
%\subsection{Disscusion about why use perceptual loss and why apply the visual masking for feature maps rather than the image}
\subsection{Comparisons between perceptual loss and $L_{1}$ loss}
\label{loss comparisons}

In this section, we will discuss the superiority of adapting perceptual loss.

To explain more efficiently, we first compare the results between $L_{1}$ and perceptual loss via directly optimizing with the original HDR images and then compare the results optimized with adaptive $\mu$-lawed HDR images. Table \ref{tabel: comparsion of loss} shows the TMQI score of perceptual and $L_{1}$ loss. We can see, the $\mathrm{TMQI_{S}}$ and BRISUQE score improves obviously, which means the perceptual loss has a very important role for structural fidelity as well as contrast, as mentioned in Section \ref{ablation studies}. Fig. \ref{fig: comparsion of loss} shows the subjective comparisons, we can see that the perceptual loss will lead to more clear details and is s good at handling the highlight regions. However, $L_{1}$ causes blurry results.

%As discuss above , we implement the visual masking to the feature maps of pretrainied VGG, and we also explorate that apply visual masking on images and then optimise with perceptual loss. Table \ref{tabel: image and feature} show the objective score comparisons and Fig \ref{fig: image and feature} show the visual comparisons.
\begin{table*}
 	\caption{\label{tabel: comparsion of loss}%
           Comparisons of  $L_{1}$ loss and perceptual loss.  Mean and standard deviation for 180 test images form three different dataset.}
	\centering
	 \begin{tabular}{|c  |c |c |c |c|c|} 
	 \hline
	 Loss Function & TMQI($\uparrow$) &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$) &BTMQI ($\downarrow$) &BRISQUE ($\downarrow$) \\ [0.5ex] 
	 \hline
	 $L_{1}$ loss  &0.7264 $\pm$ 0.2647  & 0.6614 $\pm$ 0.3449  &0.3135 $\pm$ 0.3023  & 4.9683 $\pm$  1.6459 &33.4456 $\pm$ 10.8092 \\ 
	 \hline
	Pecpetual loss   & 0.8290 $\pm$ 0.0947  & 0.8528 $\pm$ 0.1379  &0.2714 $\pm$ 0.2703 & 4.9112 $\pm$  1.6139 & 23.93 $\pm$ 9.0689\\
	 \hline
	 $L_{1}$ loss ($\mu$-law) & 0.8955 $\pm$ 0.0539 & 0.8562 $\pm$ 0.0691 & 0.5805 $\pm$ 0.2600 & 3.4688 $\pm$ 1.1094  & 27.7316 $\pm$ 8.6018\\ 
	 \hline
	Pecpetual loss ($\mu$-law)  &  \textbf{0.9152 $\pm$ 0.0484}  &\textbf{0.8926 $\pm$ 0.0628}  &\textbf{0.6382 $\pm$ 0.2483}  & \textbf{3.2477 $\pm$ 1.0442}  &\textbf{ 22.1843 $\pm$ 8.7912}\\
	 \hline
	\end{tabular}
\end{table*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[ $L_{1}$ loss: 0.8081]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1_no_ulaw/hdr_179.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Peceptual Loss: 0.8160]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual_no_ulaw/hdr_179.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$L_{1}$ loss  with $\mu$-law: 0.8878]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1/hdr_179.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Peceptual loss  with $\mu$-law: 0.8995]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual/hdr_179.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[ $L_{1}$ loss: 0.8828]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1_no_ulaw/hdr_65.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Peceptual Loss: 0.9102]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual_no_ulaw/hdr_65.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[$L_{1}$ loss  with $\mu$-law: 0.9088]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1/hdr_65.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Peceptual loss with $\mu$-law: 0.9773]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual/hdr_65.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: comparsion of loss}%
            Visual Comparisons of $L_{1}$ loss and perceptual loss. The two left columns are tested without $\mu$ law, while the two rights are with $\mu$ law. The results from $L_{1}$ loss tends to be blurry, lots of details are missing.}
\end{figure*}


\subsection{Comparison between feature contrast masking in feature maps and images}
\label{fai}
In this section, we will discuss why implementing our feature contrast masking model on feature maps rather than the image.
In this paper, we apply the masking to the feature maps of pre-trained VGG, the process is illustrated in section \ref{vml}. We also explore applying the masking model to image space, which is the traditional visual masking common practice. This is to say, implement the masking model on the HDR image and output tone mapping image, and then directly calculate the perceptual loss.
From Table \ref{tabel: image and feature}, it is clear that applying masking to feature maps has a higher score on TMQI, lower score on BTMQI and BRISQUE, which means it has more natural appearance. In detail, same as the previous experiment, thanks to the use of perceptual loss,  the $\mathrm{TMQI_{S}}$ score of image-masked resultsa is still comparable while the $\mathrm{TMQI_{N}}$ has an obvious decline. The visual results are shown in Fig. \ref{fig: image and feature} prove our inference. The feature contrast masked results is more clear and bright while the image-masked results are more blurry and dark, which means they lose the local contrast and lead to brightness distortion.
\begin{table*}
 	\caption{\label{tabel: image and feature}%
            Comparisons of applying visual masking on images and feature maps. Mean and standard deviation for 180 test images form three different dataset.
           }
	\centering
	 \begin{tabular}{|c  |c |c |c |c |c|} 
	 \hline
	 Methods & TMQI  ($\uparrow$)  &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$) & BTMQI ($\downarrow$) &BRISQUE ($\downarrow$) \\ [0.5ex] 
	 \hline
	 Image visual masking & 0.8650 $\pm$ 0.0608 & 0.8848 $\pm$ 0.0741  & 0.3787 $\pm$ 0.2749 & 3.9317 $\pm$ 1.2795  & 22.9182 $\pm$ 8.7425\\ 
	 \hline
	Feature contrast masking & \textbf{0.9250 $\pm$ 0.0438} &\textbf{0.8891 $\pm$ 0.0579} &  \textbf{0.7040 $\pm$ 0.2379} & \textbf{3.0075 $\pm$ 1.003} & \textbf{20.7904 $\pm$ 8.3566}\\
	 \hline
	\end{tabular}
\end{table*}

\begin{figure*}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Image visual masking: 0.7839]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_28.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Feature contrast masking: 0.9188]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_28.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Image visual masking: 0.8477]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_5.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Feature contrast masking: 0.9723]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_5.png}
		\end{minipage}
	}\hspace{-1pt}
          \quad
	\subfloat[Image visual masking: 0.9688]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_60.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Feature contrast masking: 0.9786]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_60.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Image visual masking: 0.8796]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Feature contrast masking: 0.9676]{
		\begin{minipage}{0.225\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_53.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: image and feature}%
         Visual Comparisons of Applying Visual Masking on images and Feature Maps. The results from image-based visual masking suffers global and local contrast distortion, which can be darker and blurry. }
\end{figure*}

%------------------------------------------------------------------------


%------------------------------------------------------------------------
%\section{Failure Case}
%During experiments, we find that our method performs not well for the extremely high dynamic range scenes, such as shadow with sunlight, which is shown in Fig. \ref{fig: failure case}.


%-------------------------------------------------------------------------
\section{Conclusions}

Tone mapping is a promising technology to display HDR images normally in SDR monitors. Traditional tone mapping methods can not handle the various scenarios well with complex parameter settings. The recent learning-based algorithms are supervised training methods, which need paired training data. They generate the labels by selecting the results with high TMQI scores or manually from the tone-mapped images produced by other tone mapping methods. However, the labels are not reliable since there are no perfectly tone mapping operators. In addition, the labels will limit the performance of the results.  In this paper, we propose a small image-specific self-supervision tone mapping network without annotated labels. We consider tone mapping from three aspects, structural fidelity of HDR images, contrast, and brightness. Based on this analysis, we first implement exposure sampling to the HDR image to generate three different exposure LDR images, which can preserve all the HDR information while compressing the dynamic range. Then an adaptive $\mu$-law is designed and applied to the HDR images for better brightness and global contrast compression. Finally, to have better structural fidelity and local contrast control, we adopt perceptual loss by applying the visual masking model to the feature maps as the loss function. We have verified that our algorithm outperforms other methods on a large-scale test set both of objective and subjective evaluations. However, during experiments, we still find that our method performs not well for the extremely high dynamic range scenes, such as shadow with sunlight, which is shown in Fig. \ref{fig: failure case}. We can find the results of these kinds of scenes tend to be a little over-exposed, the local and global contrast both suffer a loss. We think the reason could be our network is too small, so it is a lack of capacity for handling such challenging unbalanced scenarios. For future work, first, we will try to use more advanced network architecture, such as attention module and transformer, they can capture the global information effectively and can make up for the deficiency of CNN to make it more powerful. Second, we will focus on the acceleration and try to make it real-time. 

\begin{figure}[htb]
\captionsetup[subfigure]{labelformat=empty}
	\subfloat[Scene 1: 0.8078]{
		\begin{minipage}{0.45\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/failure_case/hdr_50.png}
		\end{minipage}
	}\hspace{-1pt}
	\subfloat[Scene 2: 0.8488]{
		\begin{minipage}{0.45\linewidth}
			\includegraphics[width=1\linewidth]{./figures/ablation/failure_case/hdr_105.png}
		\end{minipage}
	}\hspace{-1pt}
	\centering
	\caption{\label{fig: failure case}%
         Examples of failure case. The results are little over-exposed, and lose both global and local contrast.}
\end{figure}

\clearpage
%-------------------------------------------------------------------------
% bibtex
\bibliographystyle{eg-alpha-doi} 
\bibliography{egbibsample}      

% biblatex with biber
% \printbibliography                

%-------------------------------------------------------------------------
%\newpage




\end{document}


==> EG22_exploration.tex <==
%------------------------------------------------------------------------


\section{Explorations}
\label{explorations}
%------------------------------------------------------------------------
\subsection{Exploration of Gaussian Kernel Size}
We provide the explorations of Gaussian kernel size to figure out how the kernel size influences the results. Fig. \ref{fig: different kernels} shows the visualizations, we can find that small kernels will lead to local contrast loss. The shadow of the tree are over-enhanced, which should be darker like the real scene. Too large kernel will introduce  more computations. We choose a medium size kernel, 13$\times$13.

over enhance the detail and lead to holo artifacts while large kernels will lose some local contrast and introduce more computational cost. Medium kernel size is more suitable, in our paper, we select kernel size 13 $\times$ 13.
%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[ kernel size = 3]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_3.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[kernel size = 13]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_13.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[kernel size = 33]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_kernels/hdr_42_31.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: different kernels}%
%           Visual explorations of different gaussian kernel size. The small kernel cannot capture enough local information, and leads to local contrast loss. Too large kernel will introduce extensive calculations. We choose a medium size kernel, 13$\times$13.}
%\end{figure*}
\begin{figure}[bth]
	\centering
	\includegraphics[width=\linewidth]{./figures/results_new/kernelsize.pdf}
	\caption{\label{fig: different kernels}	
		Visual Comparison of Ablation Study. The small kernel cannot capture enough local information, and leads to local contrast loss. Too large kernel will introduce extensive calculations. We choose a medium size kernel, 13$\times$13.}
\end{figure}
%------------------------------------------------------------------------
\subsection{Exploration of Non-linearity}
\label{non-lin}
 
We also explore the influence of non-linear parameters $\alpha$ and $\beta$ as mention in Section \ref{vml}. From Fig. \ref{fig: different weights}, we can see that the $\alpha$ and $\beta$ coordinate with each other to control the local contrast. $\alpha$ controls the non-linearity of the numerator, which can emphasize the local contrast, with $\alpha$ decreasing, more details will appear. $\beta$ can adjust the non-linearity of the denominator, which can suppress large contrast regions. For better visual pleasing results, we choose $\alpha$ = 0.5 and $\beta$ = 0.5.

%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[ $\gamma$ = 0.9, $\beta$ = 0.9]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.9.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.9, $\beta$ = 0.5]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.5.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.9, $\beta$ = 0.1]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.9_0.1.png}
%		\end{minipage}
%	}\hspace{-1pt}
%           \quad
%	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.9]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.9.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[ $\gamma$ = 0.5, $\beta$ = 0.5]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.5.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.5, $\beta$ = 0.1]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.5_0.1.png}
%		\end{minipage}
%	}\hspace{-1pt}
%           \quad
%	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.9]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.9.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.5]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.5.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$\gamma$ = 0.1, $\beta$ = 0.1]{
%		\begin{minipage}{0.3\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/different_weights/hdr_127_0.1_0.1.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: different weights}%
%           Visual explorations of different weights of $\gamma$ and $\beta$.  $\gamma$ controls the non-linearity of the numerator, which can emphasize the local contrast, with $\gamma$ decreasing, more details will appear, as each column shows. $\beta$ can adjust the non-linearity of the denominator, which can suppress large contrast regions, as each row shows. $\gamma$ and $\beta$ cooperate to control the contrast.}
%\end{figure*}
\begin{figure}[bth]
	\centering
	\includegraphics[width=\linewidth]{./figures/results_new/alpha.pdf}
	\caption{\label{fig: different weights}	
		Visual explorations of different weights of $\alpha$.  $\alpha$  can control the local contrast, in order to have a natural local contrast, we select $\alpha$ = 0.5 in this paper.}
\end{figure}
%------------------------------------------------------------------------
%\subsection{Disscusion about why use perceptual loss and why apply the visual masking for feature maps rather than the image}
\subsection{Comparisons between perceptual loss and $L_{1}$ loss}
\label{loss comparisons}

In this section, we will discuss the superiority of adapting perceptual loss.

To explain more efficiently, we first compare the results between $L_{1}$ and perceptual loss via directly optimizing with the original HDR images and then compare the results optimized with adaptive $\mu$-lawed HDR images. Table \ref{tabel: comparsion of loss} shows the TMQI score of perceptual and $L_{1}$ loss. We can see, the $\mathrm{TMQI_{S}}$ and BRISUQE score improves obviously, which means the perceptual loss has a very important role for structural fidelity as well as contrast, as mentioned in Section \ref{ablation studies}. Fig. \ref{fig: comparsion of loss} shows the subjective comparisons, we can see that the perceptual loss will lead to more clear details and is s good at handling the highlight regions. However, $L_{1}$ causes blurry results.

As discuss above , we implement the visual masking to the feature maps of pretrainied VGG, and we also explorate that apply visual masking on images and then optimise with perceptual loss. Table \ref{tabel: image and feature} show the objective score comparisons and Fig \ref{fig: image and feature} show the visual comparisons.
\begin{table*}
 	\caption{\label{tabel: comparsion of loss}%
           Comparisons of  $L_{1}$ loss and perceptual loss.  Mean and standard deviation for 180 test images form three different dataset.}
	\centering
	 \begin{tabular}{|c  |c |c |c |c|c|} 
	 \hline
	 Loss Function & TMQI($\uparrow$) &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$) &BTMQI ($\downarrow$) &BRISQUE ($\downarrow$) \\ [0.5ex] 
	 \hline
	 $L_{1}$ loss  &0.7928 $\pm$ 0.2120  & 0.7456 $\pm$ 0.2712  &0.3858 $\pm$ 0.3116  & 4.7095 $\pm$ 1.6464 &31.9245 $\pm$ 10.6686 \\ 
	 \hline
	Pecpetual loss   & 0.8486 $\pm$ 0.0888  & 0.8572 $\pm$ 0.1205  &0.3543 $\pm$ 0.2891 & 4.5592 $\pm$  1.61171 & 22.3732 $\pm$ 9.1862\\
	 \hline
	 $L_{1}$ loss ($\mu$-law) & 0.8987 $\pm$ 0.0521 & 0.8553 $\pm$ 0.0682 & 0.6009 $\pm$ 0.2578  & 3.5198 $\pm$ 1.2056  & 28.2998 $\pm$ 8.9706\\ 
	 \hline
	Pecpetual loss ($\mu$-law)  &  \textbf{0.9178 $\pm$ 0.0462}  &\textbf{0.8913 $\pm$ 0.0607}  &\textbf{0.6596 $\pm$ 0.2470}  & \textbf{3.1934 $\pm$ 1.1220}  &\textbf{ 22.1773 $\pm$ 8.6294}\\
	 \hline
	\end{tabular}
\end{table*}

%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[ $L_{1}$ loss: 0.8081]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1_no_ulaw/hdr_179.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Peceptual Loss: 0.8160]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual_no_ulaw/hdr_179.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$L_{1}$ loss  with $\mu$-law: 0.8878]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1/hdr_179.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Peceptual loss  with $\mu$-law: 0.8995]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual/hdr_179.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[ $L_{1}$ loss: 0.8828]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1_no_ulaw/hdr_65.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Peceptual Loss: 0.9102]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual_no_ulaw/hdr_65.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[$L_{1}$ loss  with $\mu$-law: 0.9088]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_l1/hdr_65.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Peceptual loss with $\mu$-law: 0.9773]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_peceptual/hdr_65.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: comparsion of loss}%
%            Visual Comparisons of $L_{1}$ loss and perceptual loss. The two left columns are tested without $\mu$ law, while the two rights are with $\mu$ law. The results from $L_{1}$ loss tends to be blurry, lots of details are missing.}
%\end{figure*}

\begin{figure}[bth]
	\centering
	\includegraphics[width=\linewidth]{./figures/results_new/perceptual.pdf}
	\caption{\label{fig: comparsion of loss}	
		Visual Comparisons of $L_{1}$ loss and perceptual loss. The results from $L_{1}$ loss tends to be blurry, lots of details are missing. (Here we show the results optimised with $\mu$-law compression for a better visualization. )}
\end{figure}

\subsection{Comparison between feature contrast masking in feature maps and images}
\label{fai}
In this section, we will discuss why implementing our feature contrast masking model on feature maps rather than the image.
In this paper, we apply the masking to the feature maps of pre-trained VGG, the process is illustrated in section \ref{vml}. We also explore applying the masking model to image space, which is the traditional visual masking common practice. This is to say, implement the masking model on the HDR image and output tone mapping image, and then directly calculate the perceptual loss.
From Table \ref{tabel: image and feature}, it is clear that applying masking to feature maps has a higher score on TMQI, lower score on BTMQI and BRISQUE, which means it has more natural appearance. In detail, same as the previous experiment, thanks to the use of perceptual loss,  the $\mathrm{TMQI_{S}}$ score of image-masked resultsa is still comparable while the $\mathrm{TMQI_{N}}$ has an obvious decline. The visual results are shown in Fig. \ref{fig: image and feature} prove our inference. The feature contrast masked results is more clear and bright while the image-masked results are more blurry and dark, which means they lose the local contrast and lead to brightness distortion.
\begin{table*}
 	\caption{\label{tabel: image and feature}%
            Comparisons of applying visual masking on images and feature maps. Mean and standard deviation for 180 test images form three different dataset.
           }
	\centering
	 \begin{tabular}{|c  |c |c |c |c |c|} 
	 \hline
	 Methods & TMQI  ($\uparrow$)  &$\mathrm{TMQI_{S}}$ ($\uparrow$) & $\mathrm{TMQI_{N}}$ ($\uparrow$) & BTMQI ($\downarrow$) &BRISQUE ($\downarrow$) \\ [0.5ex] 
	 \hline
	 Image visual masking & 0.8009 $\pm$ 0.0491 & 0.7642 $\pm$ 0.0833  & 0.2532 $\pm$ 0.2215 & 4.0090 $\pm$ 0.8919& 31.5048 $\pm$ 9.7357\\ 
	 \hline
	Feature contrast masking  & \textbf{0.9248 $\pm$ 0.0432} &\textbf{0.8938 $\pm$ 0.0582} &  \textbf{0.7062 $\pm$ 0.2369} & \textbf{2.9065 $\pm$ 1.0481} & \textbf{21.2208 $\pm$ 8.5981}\\
	 \hline
	\end{tabular}
\end{table*}

%\begin{figure*}[htb]
%\captionsetup[subfigure]{labelformat=empty}
%	\subfloat[Image visual masking: 0.7839]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_28.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Feature contrast masking: 0.9188]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_28.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Image visual masking: 0.8477]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_5.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Feature contrast masking: 0.9723]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_5.png}
%		\end{minipage}
%	}\hspace{-1pt}
%          \quad
%	\subfloat[Image visual masking: 0.9688]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_60.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Feature contrast masking: 0.9786]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_60.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Image visual masking: 0.8796]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_img_masking/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\subfloat[Feature contrast masking: 0.9676]{
%		\begin{minipage}{0.225\linewidth}
%			\includegraphics[width=1\linewidth]{./figures/ablation/ours_feature_masking/hdr_53.png}
%		\end{minipage}
%	}\hspace{-1pt}
%	\centering
%	\caption{\label{fig: image and feature}%
%         Visual Comparisons of Applying Visual Masking on images and Feature Maps. The results from image-based visual masking suffers global and local contrast distortion, which can be darker and blurry. }
%\end{figure*}
\begin{figure}[bth]
	\centering
	\includegraphics[width=\linewidth]{./figures/results_new/img_masking.pdf}
	\caption{\label{fig: image and feature}	
		Visual Comparisons of Applying Visual Masking on images and Feature Maps. The results from image-based visual masking can excessively enhance local contrast, which is unnatrual.)}
\end{figure}

